String Field Theory -- A Modern Introduction

This book provides an introduction to string field theory (SFT). String theory is usually formulated in the worldsheet formalism, which describes a single string (first-quantization). While this approach is intuitive and could be pushed far due to the exceptional properties of two-dimensional theories, it becomes cumbersome for some questions or even fails at a more fundamental level. These motivations have led to the development of SFT, a description of string theory using the field theory formalism (second-quantization). As a field theory, SFT provides a rigorous and constructive formulation of string theory. The main objective is to construct the closed bosonic SFT and to explain how to assess the consistency of string theory with it. The accent is put on providing the reader with the foundations, conceptual understanding and intuition of what SFT is. After reading this book, they should be able to study the applications from the literature. The book is organized in two parts. The first part reviews the topics of the worldsheet theory that are necessary to build SFT (worldsheet path integral, CFT and BRST quantization). The second part starts by introducing general concepts of SFT from the BRST quantization. Then, it introduces off-shell string amplitudes before providing a Feynman diagrams interpretation from which the building blocks of SFT are extracted. After constructing the closed SFT, it is used to outline the proofs of several important consistency properties, such as background independence, unitarity and crossing symmetry. Finally, the generalization to the superstring is also discussed. This book grew up from lecture notes for a course given at the Ludwig-Maximilians-Universit\"at LMU (winter semesters 2017-2018 and 2018-2019). The current document is the draft of the manuscript published by Springer.

==> abstract.tex <==
\begin{abstract}
This \revname{} provides an introduction to string field theory (SFT).
String theory is usually formulated in the worldsheet formalism, which describes a single string (first-quantization).
While this approach is intuitive and could be pushed far due to the exceptional properties of two-dimensional theories, it becomes cumbersome for some questions or even fails at a more fundamental level.
These motivations have led to the development of SFT, a description of string theory using the field theory formalism (second-quantization).
As a field theory, SFT provides a rigorous and constructive formulation of string theory.

The main objective is to construct the closed bosonic SFT and to explain how to assess the consistency of string theory with it.
The accent is put on providing the reader with the foundations, conceptual understanding and intuition of what SFT is.
After reading this book, she should be able to study the applications from the literature.

The \revname{} is organized in two parts.
The first part reviews the topics of the worldsheet theory that are necessary to build SFT (worldsheet path integral, CFT and BRST quantization).
The second part starts by introducing general concepts of SFT from the BRST quantization.
Then, it introduces off-shell string amplitudes before providing a Feynman diagrams interpretation from which the building blocks of SFT are extracted.
After constructing the closed SFT, it is used to outline the proofs of several important consistency properties, such as background independence, unitarity and crossing symmetry.
Finally, the generalization to the superstring is also discussed.

This book grew up from lecture notes for a course given at the Ludwig-Maximilians-Universität LMU (winter semesters 2017--2018 and 2018--2019).
\end{abstract}


==> index_maps.tex <==
\index{adjoint|see{Euclidean, Hermitian adjoint}}

\index{bc@$bc$ CFT|see{first-order CFT, reparametrization $bc$ ghosts}}
\index{bg@$\beta\gamma$ CFT|see{first-order CFT, superconformal $\beta\gamma$ ghosts}}

\index{BRST SFT|see{covariant SFT}}

\index{closed string states!level-matching|see{level-matching}}

\index{conformal!anomaly|see{Weyl anomaly}}
\index{conformal!factor|see{Liouville field}}
\index{conformal!vacuum|see{$\mathrm{SL}(2, \C)$ vacuum}}

\index{conformal algebra!$2d$|see{Witt algebra, Virasoro algebra}}

\index{conformal isometry group|seealso{conformal Killing vector}}
\index{conformal isometry group!sphere|see{$\mathrm{SL}(2, \C)$}}

\index{covariant SFT|seealso{classical (-), free (-), quantum (-)}}

\index{Faddeev--Popov!gauge fixing|see{path integral}}

\index{factorization|see{string amplitude}}

\index{field space|seealso{path integral}}

\index{first-order CFT!Fock space|see{Hilbert space}}


\index{free covariant SFT!path integral|see{string field path integral}}

\index{fundamental vertex|seealso{closed string (-)}}

\index{G@$G$|see{spacetime ghost number}}%

\index{ghosts|see{first-order CFT, reparametrization $bc$ ghosts, superconformal $\beta\gamma$ ghosts}}

\index{mapping class group (MCG)|see{modular group}}

\index{marked Riemann surface|see{punctured Riemann surface}}

\index{metric!local rescaling|see{Weyl transformation}}

\index{Mobius@Möbius group|see{$\mathrm{SL}(2, \C)$}}

\index{puncture|see{Riemann surface}}

\index{reparametrization $bc$ ghosts|seealso{first-order CFT}}

\index{Riemann surface!g0@$g = 0$|see{Riemann sphere}}

\index{Schwinger parameter|see{propagator}}

\index{Sm@$S$-matrix|see{scattering amplitude}}

\index{spacetime momentum|seealso{scalar field CFT}}

\index{SFT|see{string field theory}}

\index{string amplitude!closed string|see{closed string amplitude}}

\index{string Feynman diagram|seealso{momentum-space SFT}}

\index{string field|seealso{string states}}
\index{string field!gauge fixing|see{Siegel gauge}}

\index{string states|seealso{closed, open (-)}}
\index{string states!on-shell|see{on-shell condition}}
\index{string states!physical|see{BRST cohomology}}


\index{superconformal $\beta\gamma$ ghosts|seealso{first-order CFT}}

\index{ultralocality|see{path integral measure}}

\index{vertex operator|seealso{string states}}
\index{vertex operator|seealso{scalar field CFT}}

\index{winding number|seealso{scalar field CFT}}

\index{worldsheet!ghosts|see{reparametrization ghosts}}
\index{worldsheet!path integral|see{Polyakov path integral}}



\index{BRST cohomology|seealso{string states}}
\index{BV formalism|see{Batalin--Vilkovisky formalism}}
\index{CFT|see{conformal field theory}}
\index{CISO|see{conformal isometry group}}
\index{ISO|see{isometry group}}
\index{OPE|see{operator product expansion}}
\index{PCO|see{picture changing operator}}



\index{$^\ddagger$|see{Euclidean adjoint}}
\index{$^\dagger$|see{Hermitian adjoint}}
\index{$^c$|see{conjugate state}}
\index{$^t$|see{BPZ conjugation}}

\index{[]@$\{ \cdots \}_g$|see{fundamental vertex}}
\index{[]@$[ \cdots ]_g$|see{string product}}

\index{x@$\mc X$|see{picture changing operator}}

\index{$\chi_g, \chi_{g,n}$|see{Euler characteristics}}

\index{$\ket{\uparrow}$|see{first-order system, vacuum}}
\index{$\ket{\downarrow}$|see{first-order system, vacuum}}


\index{$\omega_p^{g,n}$|see{$\mc P_{g,n}$ space, $p$-form}}

\index{Agn@$A_{g,n}$|see{(off-shell) string amplitude}}
\index{Rgn@$\mc R_{g,n}$|see{off-shell string amplitude contribution}}

\index{an@$\alpha_n$|see{scalar field CFT, mode expansion}}

\index{f@$f \circ$|see{CFT, finite transformation}}

\index{g@$\hat g_{ab}$|see{background metric}}
\index{g@$g_{ab}$|see{worldsheet metric}}

\index{Kg@$\mc K_g$|see{conformal Killing vector}}

\index{ker P@$\ker \adj{P_1}$|see{quadratic differential}}
\index{ker P@$\ker P_1$|see{conformal Killing vector}}

\index{I@$I(z), I^\pm(z)$|see{inversion}}

\index{Mg@$\mc M_g$|see{moduli space}}
\index{Ngh@$N_{\text{gh}}$|see{ghost number}}

\index{$\Sigma_0$|see{Riemann sphere}}
\index{$\Sigma_g, \Sigma_{g,n}$|see{Riemann surface}}

\index{Vgn@$\mc V_{g,n}$|see{fundamental vertex}}
\index{Fgn@$\mc F_{g,n}$|see{propagator region}}
\index{Vgn@$\mc V_{g,n}^{\text{1PI}}$|see{1PI vertex}}
\index{Fgn@$\mc F_{g,n}^{\text{1PR}}$|see{1PR region}}

\index{lgn@$\ell_{g,n}$|see{string product}}

\index{r@$r(\Sigma_{g,n})$|see{index}}

